Modularizing Behavioral and Architectural Crosscutting Concerns in Formal Component-Based Systems - Application to the Behavior Interaction Priority Framework

We define a method to modularize crosscutting concerns in Component-Based Systems (CBSs) expressed using the Behavior Interaction Priority (BIP) framework. Our method is inspired from the Aspect Oriented Programming (AOP) paradigm which was initially conceived to support the separation of concerns during the development of monolithic systems. BIP has a formal operational semantics and makes a clear separation between architecture and behavior to allow for compositional and incremental design and analysis of systems. We distinguish local from global aspects. Local aspects model concerns at the component level and are used to refine the behavior of components. Global aspects model concerns at the architecture level, and hence refine communications (synchronization and data transfer) between components. We formalize local and global aspects as well as their composition and integration into a BIP system through rigorous transformation primitives. We present AOP-BIP, a tool for Aspect-Oriented Programming of BIP systems, demonstrate its use to modularize logging, security, and fault tolerance in a network protocol, and discuss its possible use in runtime verification of CBSs.

==> containers.tex <==
An aspect is the single association of a pointcut expression to a joinpoint. It may also include some extra variables. However, when weaving more than one aspect, specific problems and extra considerations need to be taken into account. This section deals with explaining how to weave multiple aspects, and elaborating on ways to group them.

\subsection{Interference}
Recall that multiple concerns may happen at one joinpoint in a program.
Typically this can be seen as the \emph{tangling} phenomenon.
When secondary code is added to the joinpoint, it is possible to interfere with the existing code at the joinpoint. This behavior is called \emph{interference}. Since not all concerns are independent, interference is an important issue to study.

%\begin{example}
%Figure \ref{fig:interfere} displays the multiple weaving scenarios of two aspects $asp_1$ and $asp_2$ where:
%\begin{itemize}
%	\item $asp_1 = \tuple{B, pc, \setof{}, F_b, F_a, \setof{}}$
%	\item $asp_2 = \tuple{B, pc, \setof{}, F'_b, F'_a, \setof{}}$
%\end{itemize}
%Both aspects share the same pointcut $pc = \setof{\pcloc(\ell_1), \pcportexec(p_1)}$.
%Let $t_1$ be the transition guarded by $g_1$ labeled by $p_1$ and whose computation is $f_1$.
%Both aspects will share the same match: $m = \tuple{\setof{t_1}, \WCurrentBefore, \WCurrentAfter}$.
%According to the execution frame both $F_b$ and $F'_b$ must be prepended to $f_1$.
%$F_a$ and $F'_a$ must be appended to $f_1$.
%The four scenarios display the possible arrangements to order $F_b$, $F_b'$, $F_a$ and $F'_a$.
%The order would not be an issue if all those functions do not write to the component variables.
%For example in the case of logging, the ordering would not matter.
%However suppose $F_b = \ffunc[x := 3]$ and $F'_b = \ffunc[x := 2]$.
%The variable $x$ will be changed to either $3$ or $2$ by the end of the before section.
%This causes the original computation $f_1$ to behave non-deterministically if it depends on $x$.
%\end{example}

%\getexamples[interfere]{example-inter1, example-inter2, example-inter3, example-inter4}
%			{Interference In Atomic Components}{0.8}{2}

Defining the composition of aspects helps to deal with interference in a more predictable way.
To do so, we examine in the following sections: (1) a modular unit that groups aspects, and (2) the operations that weave multiple aspects.

\subsection{Containers}
Aspect containers encapsulate a group of aspects.
%Containers are the equivalent of an Aspect in AspectJ.
A container consists of a sequence of aspects with shared properties.
Local containers apply to local aspects. Global containers apply to global aspects.

\begin{definition}[Local Container]
A local container is a tuple $\tuple{\tuple{\aspectlocal_1, \ldots, \aspectlocal_n}, B, V}$ such that $\forall \aspectlocal_i \in  \setof{\aspectlocal_1, \ldots, \aspectlocal_n} : \aspectlocal_i$ is applied to an atomic component $B$ and has the inter-type $V$.
\end{definition}

\begin{definition}[Global Container] A global container is a tuple $\tuple{\tuple{\aspectglobal_1, \ldots, \aspectglobal_n},V'}$ where $\forall \aspectglobal_j \in \setof{\aspectglobal_1, \ldots, \aspectglobal_m} : \aspectglobal_j $ has the inter-type $V'$.
\end{definition}

Containers define an order on the aspects they encapsulate.
This helps to define the weaving order of the aspects.
Moreover, containers ensure that aspects share the same inter-type variables.
Sharing allows the inter-type to be encapsulated in the container.
Local aspects operating on different atomic components do not interfere.
In the case of local aspects, aspects are required to operate on the same atomic component encouraging encapsulation.


\subsection{Weaving Procedures}
\label{sec:weaving-procedures}
To deal with interference we propose two approaches to compose aspects.
These two approaches specify the system on which aspects match their pointcuts.
The aspects are presented in a sequence  $\tuple{asp_1, \ldots, asp_n}$ where $asp_1, \ldots, asp_n$ are all either global or local aspects.

For a local aspect $\aspectlocal = \tuple{B, pc, V, F_b, F_a, R}$ we denote $B, pc, V, \tuple{F_b, F_a, R}$ as $\aspectlocal.B$, $\aspectlocal.pc$, $\aspectlocal.V$ and $\aspectlocal.adv$, respectively.
For a global aspect $\aspectglobal = \tuple{\composite, pc', V', F'_b, F'_a}$ we denote $\composite, pc', V', \tuple{F'_b, F'_a}$ as $\aspectglobal.\composite$, $\aspectglobal.pc$, $\aspectglobal.V$ and $\aspectglobal.adv$ respectively.

\subsection*{Weave Serial}
The first compositional approach $\weaveserial$ allows the pointcut of aspect $asp_i$ where  $i \in \setof{2, \ldots, n}$ to match any changes introduced by all aspects prior to it: $asp_j$ where $\forall j: j < i$.
\begin{definition}[$\weaveserial$] Depending on the aspect type we have two operations:
\begin{itemize}
	\item The procedure $\weaveserial_\ell$ applied to a sequence of local aspects  $\tuple{asp_1, \ldots, asp_n}$ is defined as: $\composite' = \weaveserial_\ell(\composite, \tuple{asp_1, \ldots, asp_n}) = ((((\composite \weave asp_1) \weave asp_2) \weave ..) \weave asp_n)$
	\item The procedure $\weaveserial_g$ applied to a sequence of global aspects  $\tuple{asp_1, \ldots, asp_m}$ is defined as: $\composite' = \weaveserial_g(\composite, \tuple{asp_1, \ldots, asp_m}) = ((((\composite \weaveg asp_1) \weaveg asp_2) \weaveg ..) \weaveg asp_m)$
\end{itemize}
\end{definition}


\subsection*{Weave All}
The second compositional approach $\weaveall$ allows the pointcut of aspect $asp_i$ in the sequence to not match extra behavior of the advices of all prior aspects $asp_j$ where ($\forall j : j < i$).
The non-matched behavior is the added transitions from the reset locations of local aspects.
Therefore $\weaveall$ only applies to local aspects, as global advices do not introduce new interactions.

The matching of pointcuts is separate from the weaving procedure, therefore it is possible to match the joinpoints of all the sequence of aspects before we start weaving them.
The operation $\weaveall$ matches all the pointcuts of the sequence, then weaves the aspects according to their order based on their original match projected onto the new component.

Given two aspects $asp_1$ and $asp_2$, their corresponding matches on a component $\composite_0 = \pi(\gamma(\atoms))$ are: $m_1 = \pcmatch(asp_1.B, asp_1.pc)$ and $m_2 = \pcmatch(asp_2.B, asp_2.pc)$ where $asp_1.B, asp_2.B \in \atoms$.
Weaving $asp_1$ results in $\tuple{\composite_1, \tmap_1} = \fweavel(\composite_0, asp_1.B, m_1, asp_1.V, asp_1.adv)$.
The weaving of $asp_2$ needs to apply on $\composite_1$ and therefore its original match $m_2$ needs to apply to transitions in $\composite_1$ as the local weave changes the transitions.
Therefore $m_2$ is projected onto $\composite_1$ using $project(m_2, g_1)$. Which replaces the old transitions with their changes.
\[
	project(M, \tmap) = \bigcup_{t \in M} (\tmap(t))
\]
To enable weaving the $k^{th}$ aspect we need to project over all $k-1$ weaves using $\tuple{\tmap_1 \ldots, \tmap_{k - 1}}$.
\[
	follow(M, \tuple{\tmap_1, \ldots, \tmap_{k-1}}) =  \twopartdef{project(project(project(M, \tmap_1), \ldots), \tmap_{k-1})} {k - 1 > 1}
								{M} {\text{otherwise}}
\]

The $\weaveall$ for a sequence of $n$ local aspects on a composite component $\composite_0$ is defined as $\tuple{\composite_n, \tmap_n} = \weaveall(\composite_0, \tuple{asp_1, \ldots, asp_n})$ such that: 
\begin{align*}
\intertext{$\forall i \in \setof{1, \ldots, n}$: }
	\tuple{\composite_i, \tmap_i} &= \fweaveg(\composite_{i - 1}, follow(M_i, \tuple{\tmap_1, \ldots, \tmap_{i-1}}), asp_i.V, asp_i.adv)\\
	M_i &= \pcmatchg(\composite_0, asp_i.pc)
\end{align*}

\subsection*{Discussion}
The reset location in local advices is designed to cause the component to directly move to a location given a guard. In the case of $\weaveserial$, the reset location only incorporates advices of aspects that are woven after it, but not before.
The $\weaveall$ provides finer tuning on the behavior of a reset location by making reset location not incorporate advices of subsequent aspects.
This provides another way to manage interference between various aspects implementing reset location.

For both $\weaveserial$ and $\weaveall$, the reset location can cause a component to execute a \code{before} advice without its corresponding \code{after}.
This scenario typically happens when a reset location is woven on an earlier execution frame than an \code{after} advice.
Given a sequence of aspects $\tuple{a_1, \ldots, a_n}$ and two aspects $a_i$ and $a_j$ such that $i < j$.
Let the frame of $a_i$'s joinpoints be $\tuple{i_s, i_e}$ and that of  $a_j$'s joinpoints be $\tuple{j_s, j_e}$. 
If $j_s \prec i_e$ and $i_e \prec j_e$, a reset location in $a_i.adv$ would be woven prior to $j_e$.
Therefore, $j_e$ is not executed along with any after advice woven onto it.
It is possible to avoid the scenario by composing aspects differently.
Two example compositions involve:
\begin{enumerate}
    \item Ordering aspects by their execution frames;
    \item Splitting an aspect into two aspects such that (a) one contains a reset location only advice and (b) another contains the \code{before} and \code{after} advice only. Then, the ones with reset locations are  woven first, the rest are woven with $\weaveserial$. This ensures all \code{before} and \code{after} apply to all reset locations.
\end{enumerate}

%\getexamples[inter]{compose/c1, compose/c2, compose/c3, compose/c4, compose/c5, compose/c6}
%			{Weaving Procedures}{0.8}{2}
%\begin{example}
%\rfig{fig:inter} shows the different results obtained by composing two aspects $a$ and $a'$ onto an atomic component.
%The joinpoints are provided by matching $a.pc = \setof{\pcloc(\ell_0), \pcportexec(p_2)}$ and $a'.pc = \setof{\pcloc(\ell_1)}$.
%The corresponding advices are $a.adv = \tuple{F_b, F_a, \setof{\tuple{\ell_0, \btrue}}}$ and $a'.adv = \tuple{F'_b, F'_a, \setof{}}$.
%\begin{itemize}
%	\item
%\rfig[a]{fig:inter} and \rfig[b]{fig:inter} show the weaving of each aspect individually.
%When weaving the two aspects into one system, overlap causes interference.
%Let $m$ denote the match of $a$, $m'$ denote the match of $a'.pc$ and $t_5$ the transition guarded by $g_5$.
%The transition $t_5$ is both in the joinpoint of $m$ and $\WGetP(m')$.
%Depending on the order of weave the newly created reset location could also be found in $m'$ as it is outbound from $\ell_1$.
%	\item
%\rfig[c]{fig:inter} and \rfig[d]{fig:inter} show the $\weaveserial_\ell$ operation.
%	\begin{enumerate}
%		\item 
%\rfig[c]{fig:inter} presents the serial weave on $a$ followed by $a'$. The weave of $a$ results in $\tuple{\composite_1, g_1}$. $\composite_1$ is shown in \rfig[a]{fig:inter}.
%Upon weaving $a'$ its pointcut will match the reset location as it is outbound from $\ell_1$ and will therefore prepend $F'_a$ to it.
%The pointcut will also match $g_1(t_5)$ as it is inbound, therefore it appends $F'_b \aopclear'$ to its existing function which is now $F_b f_5 F_a \aopset$ since $a$ was already woven.
%		\item
%\rfig[d]{fig:inter} presents the serial weave on $a'$ followed by $a$. The weave of $a'$ results in $\tuple{\composite'_1, g'_1}$. The component is shown in \rfig[b]{fig:inter}.
%Upon weaving $a$ the pointcut will match $g'_1(t_5)$. Its function $f_5 F'_b \aopclear'$ is then appended with $F_a \aopset$.
%Additionally the reset location is then added guarded by $b \land \btrue$.
%	\end{enumerate}
%	\item
%\rfig[F]{fig:inter} show the $\weaveall$ operation and how it differs from the $\weaveserial$.
%The pointcut of $a'$ will always match against the original component, matching always the transition guarded by $g_5$.
%The $\weaveall$ projects the match.
%The new match result will be $t_5$ if $a'$ is woven first or $g_1(t_5)$ if $a$ is woven first.
%The joinpoint will therefore not contain the reset location in both cases.
%The order of the aspects still define the order of the advices woven onto overlapping transitions.
%\rfig[e]{fig:inter} displays the different advices order.

%\end{itemize}
%\end{example}


==> tikz/aopvars.tex <==
\node[var] (x) at ( $(c1.north east) + (-0.5, -0.5)$) []  {x};
\node[var, color=\colorhigh] (aop)  [left=of x, shift={(0.5,0)}]  {$\aopvar$};	


==> tikz/compose/aopvars.tex <==
\node[var] (x) at ( $(c1.north east) + (-0.5, -0.5)$) []  {x};
\node[var, color=\colorhigh] (b1)  [left=of x, shift={(0.5,0)}]  {$b$};	
\node[var, color=\colorhigh] (b2)  [left=of b1, shift={(0.5,0)}]  {$b'$};	


==> tikz/toverlay.tex <==
\node[above=of t5, shift={(-0.6, -0.9)}] () {$\textbf t_5$};
\node[left= of t0, shift={(+1.4, -0.1)}] () {$\textbf t_0$};
\node[right=of t1, shift={(-0.9, 0)}] () {$\textbf t_1$};
\node[left= of t2, shift={(+1.4, -0.1)}] () {$\textbf t_2$};
\node[right=of t3, shift={(-1.2, 0)}] () {$\textbf t_3$};
\node[right=of t4, shift={(-2, 0)}] () {$\textbf t_4$};

